TERRA: Beam Management for Outdoor mm-Wave Networks

mm-Wave communication systems use narrow directional beams due to the spectrum's characteristic nature: high path and penetration losses. The mobile and the base station primarily employ beams in line of sight (LoS) direction and when needed in non-line of sight direction. Beam management protocol adapts the base station and mobile side beam direction during user mobility and to sustain the link during blockages. To avoid outage in transient pedestrian blockage of the LoS path, the mobile uses reflected or NLoS path available in indoor environments. Reflected paths can sustain time synchronization and maintain connectivity during temporary blockages. In outdoor environments, such reflections may not be available and prior work relied on dense base station deployment or co-ordinated multi-point access to address outage problem. Instead of dense and hence cost-intensive network deployments, we found experimentally that the mobile can capitalize on ground reflection. We developed TERRA protocol to effectively handle mobile side beam direction during transient blockage events. TERRA avoids outage during pedestrian blockages 84.5 $\%$ of the time in outdoor environments on concrete and gravel surfaces. TERRA also enables the mobile to perform a soft handover to a reserve neighbor base station in the event of a permanent blockage, without requiring any side information, unlike the existing works. Evaluations show that TERRA maintains received signal strength close to the optimal solution while keeping track of the neighbor base station.

==> switching_evaluation.tex <==
\section{Comment on Base Station Density and Switching Policy}
\subsubsection{Base Station Density}

% Due to high penetration loss in the mm-wave bands, pedestrians moving across a directional communication link between a base station and mobile obstruct the radiation. In such blockage events, the signal strength at mobile drops significantly. Studies have shown that such blockage events can last for a few hundred milliseconds. To revive the communication and maintain the user experience under the blockage, the mobile needs to switch to an alternate base station in the outdoor environment. 
% In indoors, handover is not necessary as there is a possibility of establishing the link with the same base station via NLoS directions during blockage events.


\red{First you should refer to papers that propose switching base stations every time there is a pedestrain blockage. Then you should say, in order to do this } \sout{During pedestrian blockage events, to quickly switch base stations,} the mobile must have a neighbor base station in reserve at any location in the coverage area. \sout{Search takes quite long time, so instant switching is not possible.} Dense network deployment is \sout{also} necessary, since at least two base stations need to be visible to the mobile at any given location in the coverage area. 
Suppose a network deployment where base station locations follow a homogeneous spatial Poisson process, 
% we study the base station density required for a mobile to listen to multiple base stations at any given location. Suppose that 
where each base station has a range $R$. \sout{Mobile can listen to a base station if it is within distance $R$ from its position.} 
Since mm-wave cells have a smaller coverage area compared to sub-6GHz Omni-directional cells, we study \sout{coverage radius} \red{ranges} from 100 to 500 m. Fig.~\ref{bsdensity} presents the number of base stations per square kilometer versus the probability of finding at least two base stations in a region of radius $R$. The dashed line in Fig. \ref{bsdensity} represents the base density ($\lambda$) necessary for the visibility of two or more base stations at any point in $90\%$ of the serving base station's coverage area. 
% As the coverage area of an individual base station decreases, the base density necessary to overcome blockage impairments increases. 
A smaller range is characteristic of base stations in mm-wave bands due to high path loss. 
% However, pedestrian blockage demands even higher dense deployments.
About 30 base stations per square kilometer are required when base stations have a range of 100 m. Such highly dense deployments are expensive and atypical in rural and semi-urban environments. Even for base stations with a 300 m range, four base stations per square kilometer are necessary.
\begin{figure}
    \centering
    \includegraphics[width=.6\linewidth]{figures/base_station_density.pdf}
    \caption{Base Station Density for mm-wave deployments}
    \label{bsdensity}
\end{figure}


\red{The section on Switching Policy can be omitted since it does not really present any new results
or viewpoints.}
% \subsection{Switching Policy}

% If not for a blockage event, a mobile usually switches base stations only if it moves to the edge of a cell. The mm-wave deployments are dense. At cell edge, a mobile has multiple base stations to hand. The mobile requires holistic information to make the right switching decision. Knowledge of the radio environments of all the neighbor base stations, the direction of user motion, and possibly the destination of the user too.

%  Either mobile makes measurements or the network needs to share  information with mobile to apprehend the radio environment of all the neighbor base stations.
% The Mobile's receiver listens to each base station to make measurements.  First, the mobile performs a receive beam scan to listen to each base station and later adapts the beam as the user moves.

% For example, say mobile found two neighbor base stations after the conclusion of the directional search. The mobile now keeps track of three base station beams, one serving, and two neighbors. 
% The mobile repeatedly toggles the frequency of the radio receiver, adapts beams, and measures signal strengths. 

%  This process of keeping tracking of multiple base stations is energy-intensive. 
% With the number of base stations, the number of measurements increase linearly. To measure signal strengths on $K$ neighbor beams, for each one of the  $N$ neighbor base stations, mobile requires $K*(N)$ opportunities. 
% However, in case the visiting time for a base station exceeds the beam coherence time \cite{beamsurfer}, mobile cannot track of that base station. If mobile loses track of serving base station, hard handover is imminent. 
% Losing track of a neighbor base station requires a spatial scan to re-acquire. 

% For the network to assist mobile in this process, all the co-located base stations need to communicate with each other and share relevant information.
% Such communication requires either a backhaul link or a side-channel. Finally, the serving base station has to forward information to the mobile as only it can directly communicate with mobile.

% To use motion related information for handover decisions, the mobile must rely on the out-of-the-band information from the sensors. Predicting the user mobility with in-band and out of the information available to mobile is both time-consuming and energy-intensive. Also, the walking user may aimlessly handle the mobile, in that case, motion prediction is hard.

% Machine Learning based methods attempt to use historical data to make future switching decisions.
% It is well known that reliable inference requires large amount of data. 
% Generalizing the data driven models, to date, is a major area of research. 




